What Variables Affect Out-of-Distribution Generalization in Pretrained Models?

Embeddings produced by pre-trained deep neural networks (DNNs) are widely used; however, their efficacy for downstream tasks can vary widely. We study the factors influencing transferability and out-of-distribution (OOD) generalization of pre-trained DNN embeddings through the lens of the tunnel effect hypothesis, which is closely related to intermediate neural collapse. This hypothesis suggests that deeper DNN layers compress representations and hinder OOD generalization. Contrary to earlier work, our experiments show this is not a universal phenomenon. We comprehensively investigate the impact of DNN architecture, training data, image resolution, and augmentations on transferability. We identify that training with high-resolution datasets containing many classes greatly reduces representation compression and improves transferability. Our results emphasize the danger of generalizing findings from toy datasets to broader contexts.

==> figures_latex/high_resolution_main_results.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/main_results/imagenet/resnet50.png}
        \caption{ResNet50, SL}
        \label{fig:resnet50}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/main_results/imagenet/resnet50_swav.png}
        \caption{ResNet50, SwAV}
        \label{fig:resnet50_swav}
    \end{subfigure}
    \\
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/main_results/imagenet/convnext.png}
        \caption{ConvNeXt, SL}
        \label{fig:convnext}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/main_results/imagenet/dino.png}
        \caption{ViT-B, DINO}
        \label{fig:dino}
    \end{subfigure}
    \\
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/main_results/imagenet/mae.png}
        \caption{ViT-B, MAE}
        \label{fig:mae}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/main_results/imagenet/mugs.png}
        \caption{ViT-B, Mugs}
        \label{fig:mugs}
    \end{subfigure}
    \\
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/main_results/imagenet/vit.png}
        \caption{ViT-B, SL}
        \label{fig:vit}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/main_results/imagenet/swin.png}
        \caption{Swin-B, SL}
        \label{fig:swin}
    \end{subfigure}
    \caption{The tunnel effect analysis for various SL and SSL models. %Shaded area denotes the tunnel when present. Various large-scale DNNs exhibit shorter tunnel (subfig. c-h) or no tunnel (subfig. a,b).
    Large-scale DNNs do not exhibit the tunnel effect.
    }
    \label{fig:sl_ssl_results}
\end{figure}


==> figures_latex/id_ood_align_stem.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.65\linewidth]{figures/id_ood_align_stem.png}
    \caption{\textbf{Stem.} This figure exhibits ID OOD Alignment computed across stems and averaged across OOD datasets. This is based on models trained on ImagerNet-100 (ID) with $32\times 32$ and $224\times 224$ resolutions. For CNNs, the stem represents kernel size ($3\times 3$ and $7\times 7$) at the stem layer whereas, for ViTs, it is patch size ($8 \times 8$).

    }
    \label{fig:ood_retained_stem}
\end{figure}

==> figures_latex/resnet_ood_aug.tex <==

\begin{figure}[t]
    \centering
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/resnet18_ood_32_aug.png}
         \caption{ResNet-18 ($32 \times 32$)}
         \label{fig:resnet18_ood_aug_32}
     \end{subfigure}
     % \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/resnet18_ood_224_aug.png}
         \caption{ResNet-18 ($224 \times 224$)}
         \label{fig:resnet18_ood_aug_224}
     \end{subfigure}
     
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/resnet34_ood_32_aug.png}
         \caption{ResNet-34 ($32 \times 32$)}
         \label{fig:resnet34_ood_aug_32}
     \end{subfigure}
    % \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/resnet34_ood_224_aug.png}
         \caption{ResNet-34 ($224 \times 224$)}
         \label{fig:resnet34_ood_aug_224}
     \end{subfigure}
     
        \caption{
        \textbf{The OOD linear probe accuracy for ResNets trained on ImageNet-100 (ID) with image augmentations}. High resolution images ($224\times 224$) exhibit lower drops in OOD accuracy (i.e., weaker tunnel effect) than low resolution images ($32\times 32$).
        }
        \label{fig:resnet_ood_aug}
\end{figure}


==> figures_latex/resnet_ood_no_aug.tex <==

\begin{figure}[t]
    \centering
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/resnet18_ood_32_no_aug.png}
         \caption{ResNet-18 ($32 \times 32$)}
         \label{fig:resnet18_ood_no_aug_32}
     \end{subfigure}
     % \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/resnet18_ood_224_no_aug.png}
         \caption{ResNet-18 ($224 \times 224$)}
         \label{fig:resnet18_ood_no_aug_224}
     \end{subfigure}
     
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/resnet34_ood_32_no_aug.png}
         \caption{ResNet-34 ($32 \times 32$)}
         \label{fig:resnet34_ood_no_aug_32}
     \end{subfigure}
    % \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/resnet34_ood_224_no_aug.png}
         \caption{ResNet-34 ($224 \times 224$)}
         \label{fig:resnet34_no_ood_aug_224}
     \end{subfigure}
     
        \caption{
            \textbf{The OOD linear probe accuracy for ResNets trained on ImageNet-100 (ID) without image augmentations}. High resolution images ($224\times 224$) exhibit lower drops in OOD accuracy (i.e., weaker tunnel effect) than low resolution images ($32\times 32$).
        }
        \label{fig:resnet_ood_no_aug}
\end{figure}


==> figures_latex/tunnel_effect_by_resolution.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width = 0.65\linewidth]{figures/vgg_tunnel.png}
    %{figures/main_results/4.3/vgg13/dimension_comparision_224.png}
    
  \caption{The tunnel effect causes impaired OOD generalization for linear probes trained on embeddings from later layers in overparameterized DNNs; however, past work has only studied DNNs trained on $32\times32$ images. \textbf{Surprisingly, when a VGG-11 with exactly the same number of parameters is trained on the same samples at high resolution $\mathbf{(224\times224)}$, OOD performance continually increases as a function of layers and the tunnel disappears, whereas the tunnel effect is strongly exhibited (layer 8-10) when it is trained on $\mathbf{32\times32}$ images.} The layer at which linear probe accuracy reaches $\geq 95\%$ of the final accuracy evaluated on ID dataset marks the start of the tunnel (layer 8).
  Our work helps explain why many methods that are performant on toy datasets fail to scale. 
  %\yh{We need to indicate tunnel for 32x32 in the figure based on ID accuracy. Are all models trained for same number of epochs?}} 
  %The tunnel effect has profound implications across deep learning if true. In this paper, we verify that it occurs for DNNs trained with low-resolution images, but that DNNs trained on high-resolution images do not exhibit this effect. Our work helps explain why many results on datasets such as CIFAR-10 do not generalize to ImageNet-1K and other higher-resolution datasets.
  %\yh{single fig will look better here. you may combine both figure where all $32\times 32$ curves are solid ($-$) and $224\times 224$ curves are dotted or broken ($--$) or vice versa. Also you need to increase x and y axis labels and ticks.}
  }
  \label{fig:tunnel_effect_by_resolution}
\end{figure}

==> figures_latex/vgg11_data_amount.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/data_amount/different_classes.png}
        \caption{\# Classes (no aug)\label{fig:vgg11_different_class}}        
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/data_amount/different_classes_aug.png}
        \caption{\# Classes (aug)\label{fig:vgg11_different_class_aug}}        
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/data_amount/different_samples.png}
        \caption{\# Samples (no aug)\label{fig:vgg11_different_samples}}        
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/data_amount/different_samples_aug.png}
        \caption{\# Samples (aug) \label{fig:vgg11_different_samples_aug}}        
    \end{subfigure}
    \caption{%\textbf{Impact of varied classes and samples per class on the tunnel effect.}
    \textbf{Training on more classes greatly reduces the tunnel effect, whereas increasing dataset size has less impact.}
    %We show normalized OOD accuracy from linear probes applied to VGGm-11 trained on $32\times 32$ images from ImageNet-100. %where the composition of the training data is varied based on the number of classes or samples. 
    %Training on more classes reduces the tunnel effect whereas training on more samples per class has a little impact.
    \textbf{(a)} and \textbf{(b)} Results with a fixed number of samples but a varied number of classes. \textbf{(c)} and \textbf{(d)} Results with a fixed number of classes but a varied number of samples per class.  
    }
    \label{fig:vgg11-sample-size}
\end{figure}


==> figures_latex/vgg11_data_amount_aug.tex <==
\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/data_amount/different_classes_aug.png}
        \caption{Impact of number of classes}
        \label{fig:vgg11_different_class_aug}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/data_amount/different_samples_aug.png}
        \caption{Impact of number of samples per class}
        \label{fig:vgg11_different_samples_aug}
    \end{subfigure}
    \caption{Normalized OOD accuracy from linear probes applied to VGGm-11 architectures trained on $32\times 32$ images from ImageNet-100 \textbf{with augmentation}, where the composition of the training data is varied based on the number of classes or samples. Training on more classes reduces the tunnel effect whereas training on more samples per class has less impact on the tunnel effect. \textbf{(a)} Results with a fixed number of samples but varying the number of classes. \textbf{(b)} Results with a fixed number of classes but varying sample counts per class.  
    }
    \label{fig:vgg11-sample-size_aug}
\end{figure}


==> figures_latex/vgg_17_accuracy_bar_id.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.7\linewidth]{figures/vgg17_bar.png}
    \caption{\textbf{ID Datasets.} The figure shows the trend of better final OOD accuracy as the ID dataset contains more classes or sample data per class.  This figure exhibits the last layer ID and OOD accuracy of the VGG17 model trained on CIFAR-10, CIFAR-100, and ImageNet-100 with augmentation. }
    \label{fig:vgg17_ids_bar}
\end{figure}

==> figures_latex/vgg_mp.tex <==

\begin{figure}[t]
    \centering
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/vgg11_ood_32_no_aug_tunnel.png}
         \caption{VGGm-11 with max-pool}
         \label{fig:vgg11_ood_no_aug_with_mp_32}
     \end{subfigure}
     % \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/vgg11_ood_32_no_aug_wo_mp.png}
         \caption{VGGm-11 without max-pool}
         \label{fig:vgg11_ood_no_aug_no_mp_32}
     \end{subfigure}
     
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/vgg17_ood_32_no_aug_tunnel.png}
         \caption{VGGm-17 with max-pool}
         \label{fig:vgg17_ood_no_aug_with_mp_32}
     \end{subfigure}
    % \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/vgg17_ood_32_no_aug_wo_mp.png}
         \caption{VGGm-17 without max-pool}
         \label{fig:vgg17_ood_no_aug_no_mp_32}
     \end{subfigure}
     
        \caption{
            \textbf{The OOD linear probe accuracy for VGGm models with and without max-pool in first 2 stages}. The models are trained on ImageNet-100 (ID) with $32\times 32$ image resolution in \textbf{augmentation-free settings}. VGGm models without max-pool create shorter tunnels than the ones created by VGGm models with max-pool.
        }
        \label{fig:vgg_ood_mp}
\end{figure}


==> figures_latex/vgg_mp_aug.tex <==

\begin{figure}[t]
    \centering
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/vgg11_ood_32_aug_tunnel.png}
         \caption{VGGm-11 with max-pool}
         \label{fig:vgg11_ood_aug_with_mp_32}
     \end{subfigure}
     % \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/vgg11_ood_32_aug_wo_mp.png}
         \caption{VGGm-11 without max-pool}
         \label{fig:vgg11_ood_aug_no_mp_32}
     \end{subfigure}
     
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/vgg17_ood_32_aug_tunnel.png}
         \caption{VGGm-17 with max-pool}
         \label{fig:vgg17_ood_aug_with_mp_32}
     \end{subfigure}
    % \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/vgg17_ood_32_aug_wo_mp.png}
         \caption{VGGm-17 without max-pool}
         \label{fig:vgg17_ood_aug_no_mp_32}
     \end{subfigure}
     
        \caption{
            \textbf{The OOD linear probe accuracy for VGGm models with and without max-pool in first 2 stages}. The models are trained on ImageNet-100 (ID) with $32\times 32$ image resolution while using \textbf{augmentations}. VGGm models without max-pool create shorter tunnels than the ones created by VGGm models with max-pool.
        }
        \label{fig:vgg_ood_mp_aug}
\end{figure}


==> figures_latex/vgg_ood_aug.tex <==

\begin{figure}[t]
    \centering
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/vgg11_ood_32_aug.png}
         \caption{VGGm-11 ($32 \times 32$)}
         \label{fig:vgg11_ood_aug_32}
     \end{subfigure}
     % \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/vgg11_ood_224_aug.png}
         \caption{VGGm-11 ($224 \times 224$)}
         \label{fig:vgg11_ood_aug_224}
     \end{subfigure}
     
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/vgg17_ood_32_aug.png}
         \caption{VGGm-17 ($32 \times 32$)}
         \label{fig:vgg17_ood_aug_32}
     \end{subfigure}
    % \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/vgg17_ood_224_aug.png}
         \caption{VGGm-17 ($224 \times 224$)}
         \label{fig:vgg17_ood_aug_224}
     \end{subfigure}
     
        \caption{
        \textbf{The OOD linear probe accuracy for VGGm models trained on ImageNet-100 (ID) with image augmentations}. High resolution images ($224\times 224$) exhibit much lower drops in OOD accuracy (i.e., weaker tunnel effect) than low resolution images ($32\times 32$).
        }
        \label{fig:vgg_ood_aug}
\end{figure}


==> figures_latex/vgg_ood_no_aug.tex <==

\begin{figure}[t]
    \centering
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/vgg11_ood_32_no_aug.png}
         \caption{VGGm-11 ($32 \times 32$)}
         \label{fig:vgg11_ood_no_aug_32}
     \end{subfigure}
     % \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/vgg11_ood_224_no_aug.png}
         \caption{VGGm-11 ($224 \times 224$)}
         \label{fig:vgg11_ood_no_aug_224}
     \end{subfigure}
     
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/vgg17_ood_32_no_aug.png}
         \caption{VGGm-17 ($32 \times 32$)}
         \label{fig:vgg17_ood_no_aug_32}
     \end{subfigure}
    % \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/vgg17_ood_224_no_aug.png}
         \caption{VGGm-17 ($224 \times 224$)}
         \label{fig:vgg17_no_ood_aug_224}
     \end{subfigure}
     
        \caption{
            \textbf{The OOD linear probe accuracy for VGGm models trained on ImageNet-100 (ID) without image augmentations}. High resolution images ($224\times 224$) exhibit much lower drops in OOD accuracy (i.e., weaker tunnel effect) than low resolution images ($32\times 32$).
        }
        \label{fig:vgg_ood_no_aug}
\end{figure}


==> figures_latex/vit_ood_augmentation.tex <==

\begin{figure}[t]
    \centering
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/vit_tiny_ood_32_aug.png}
         \caption{ViT-T ($32 \times 32$)}
         \label{fig:vit-T_ood_aug_32}
     \end{subfigure}
     % \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/vit_tiny_ood_224_aug.png}
         \caption{ViT-T ($224 \times 224$)}
         \label{fig:vit-T_ood_aug_224}
     \end{subfigure}
     
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/vit_small_ood_32_aug.png}
         \caption{ViT-T+ ($32 \times 32$)}
         \label{fig:vit-T+_ood_aug_32}
     \end{subfigure}
    % \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/vit_small_ood_224_aug.png}
         \caption{ViT-T+ ($224 \times 224$)}
         \label{fig:vit-T+_ood_aug_224}
     \end{subfigure}
     
        \caption{
        \textbf{The OOD linear probe accuracy for ViTs trained on ImageNet-100 (ID) with image augmentations}. Both low resolution ($32\times 32$) and high resolution ($224\times 224$) images do not exhibit large drops in OOD accuracy (i.e., much weaker tunnel effect).
        }
        \label{fig:vit_ood_aug}
\end{figure}


==> figures_latex/vit_ood_no_augmentation.tex <==

\begin{figure}[t]
    \centering
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/vit_tiny_ood_32_no_aug.png}
         \caption{ViT-T ($32 \times 32$)}
         \label{fig:vit-T_ood_no_aug_32}
     \end{subfigure}
     % \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/vit_tiny_ood_224_no_aug.png}
         \caption{ViT-T ($224 \times 224$)}
         \label{fig:vit-T_ood_no_aug_224}
     \end{subfigure}
     
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/vit_small_ood_32_no_aug.png}
         \caption{ViT-T+ ($32 \times 32$)}
         \label{fig:vit-T+_ood_no_aug_32}
     \end{subfigure}
    % \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/vit_small_ood_224_no_aug.png}
         \caption{ViT-T+ ($224 \times 224$)}
         \label{fig:vit-T+_no_ood_aug_224}
     \end{subfigure}
     
        \caption{
            \textbf{The OOD linear probe accuracy for ViTs trained on ImageNet-100 (ID) without image augmentations}. Unlike low resolution images ($32\times 32$), high resolution images ($224\times 224$) exhibit large drops in OOD accuracy (i.e., stronger tunnel effect).
        }
        \label{fig:vit_ood_no_aug}
\end{figure}


==> figures_latex/vit_resnet.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/vgg17_ood_32_no_aug_tunnel.png}
        \caption{Resolution $32\times 32$}
        \label{fig:vgg_17_tunnel_res_32}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/vgg17_ood_224_no_aug_tunnel.png}
        \caption{Resolution $224\times 224$}
        \label{fig:vgg_17_tunnel_res_224}
    \end{subfigure}
    \caption{\textbf{High resolution images $(\mathbf{224\times 224})$ create \emph{shorter tunnel} (layer 13-16) than the one (layer 9-16) created by low resolution images $(\mathbf{32\times 32})$.} Gray shaded area denotes the tunnel.
    The layer after which OOD linear probe accuracy degrades marks the start of the tunnel (denoted by gray dotted vertical line).
    We use the over-parameterized VGGm-17 model and keep the number of parameters (20.08M) exactly same for both high- and low-resolutions. We train VGGm-17 models on ImageNet-100 - a subset (100 classes and 126K training samples) of ImageNet-1K, as ID dataset in augmentation-free settings.
    }
    \label{fig:vit_resnet}
\end{figure}

==> tables/acc_ood_transfer.tex <==
\begin{table}[t!]
  \caption{\textbf{Out-of-distribution (OOD) Results.} We perform linear evaluations on 8 different OOD datasets and report the best top-1 accuracy ($\%$). The models are trained on ImageNet-100 (a subset of ImageNet-1K) as an in-distribution (ID) dataset. %VGGm denotes modified VGG without two FC layers before the final layer.
  The positive $\%$ value within the Augmentation section signifies a $\%$ gain in performance, while a negative $\%$ value indicates a $\%$ decline in performance due to augmentation in comparison with the performance without augmentation.
   }
  \centering
  \resizebox{\linewidth}{!}{
  \begin{tabular}{lcc|cccccccc|c}
     \hline
     \multicolumn{1}{c}{\textbf{Model}} &
     \multicolumn{1}{c}{\textbf{Image}} &
     \multicolumn{1}{c|}{\textbf{ID}} &
     \multicolumn{9}{c}{\textbf{Transfer}} \\
      & \textbf{Size} & \textbf{ImageNet} & \textbf{NINCO} & \textbf{ImageNet-R} & \textbf{CUB} & \textbf{Aircrafts} & \textbf{Flowers} & \textbf{Pets} & \textbf{CIFAR}  & \textbf{STL} & \textbf{Avg. ($\pm$ Std.)} \\
     \hline
     \textcolor{orange}{\emph{\textbf{No Aug}}} & & & & & & & & & & & \\
     ViT-T & $32^{2}$ & $36.48$ & $47.62$ & $11.22$ & $21.45$ & $11.46$ & $39.41$ & $27.12$ & $39.67$  & $60.63$ & $32.32 (\pm16.45)$ \\
           & $224^{2}$ & $62.50$ & $54.42$ & $11.25$ & $16.15$ & $9.15$ & $26.47$ & $39.98$ & $33.11$  & $65.31$ & $31.98 (\pm19.08)$ \\
     ViT-T+ & $32^{2}$ & $35.64$ & $46.68$ & $10.68$ & $19.00$ & $10.98$ & $35.59$ & $24.83$ & $37.68$  & $59.77$ & $30.65 (\pm16.33)$ \\
            & $224^{2}$ & $59.38$ & $50.59$ & $8.68$ & $11.94$ & $7.05$ & $21.76$ & $33.82$ & $30.19$  & $59.81$ & $27.98 (\pm18.27)$ \\
     %\hline %%%%%%%%%%%%%%%%%%%%%%%
     VGGm-11 & $32^{2}$ & $52.22$ & $51.53$ & $15.22$ & $17.62$ & $16.32$ & $40.78$ & $39.68$ & $43.41$  & $68.86$ & $36.68 (\pm17.91)$ \\
            & $224^{2}$ & $78.74$ & $59.78$ & $19.02$ & $17.78$ & $17.64$ & $41.96$ & $63.86$ & $38.55$  & $77.60$ & $42.02 (\pm21.74)$ \\
     VGGm-17 & $32^{2}$ & $52.02$ & $31.80$  & $8.43$  & $6.94$  & $3.99$ & $15.00$ & $28.07$ & $24.21$  & $60.42$ & $22.36 (\pm17.31)$ \\
            & $224^{2}$ & $80.28$ & $50.51$ & $17.52$ & $12.15$ & $9.51$ & $25.98$ & $53.15$ & $32.30$  & $77.94$ & $34.88 (\pm22.30)$ \\
     ResNet-18 & $32^{2}$ & $34.38$ & $24.66$ & $5.68$  & $4.47$ & $4.86$ & $9.71$  & $16.87$ & $20.05$  & $48.69$ & $16.87 (\pm13.95)$ \\
               & $224^{2}$& $68.80$ & $54.85$ & $18.80$ & $21.06$ & $17.28$ & $43.73$& $53.28$ & $38.56$  & $74.46$ & $40.25 (\pm19.12)$ \\
     %%%%%%
     ResNet-34 & $32^{2}$ & $32.10$ & $24.40$ & $4.15$ & $4.73$ & $4.92$ & $9.51$ & $13.63$ & $18.50$  & $45.61$ & $15.68 (\pm13.18)$ \\
               & $224^{2}$ & $68.86$ & $52.98$ & $15.02$ & $17.02$ & $15.03$ & $32.06$ & $49.77$ & $33.48$  & $71.90$ & $35.91 (\pm19.46)$ \\
     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
     \hline
     \textcolor{orange}{\emph{\textbf{Aug}}} & & & & & & & & & & & \\
%      ViT-T & $32^{2}$ & $35.28$ & $49.40$ & $11.48$ & $22.11$ & $10.89$ & $41.47$ & $24.94$ & $40.25$  & $60.18$ & $32.59 (\pm16.83)$ \\
%            & $224^{2}$ & $60.72$ & $66.75$ & $17.45$ & $35.31$ & $17.04$ & $60.88$ & $51.32$ & $43.39$  & $74.29$ & $45.80 (\pm20.17)$ \\
%      ViT-T+ & $32^{2}$ & $41.14$ & $54.08$ & $13.25$ & $24.15$ & $11.49$ & $42.55$ & $30.09$  & $44.27$ & $64.50$ & $35.55 (\pm17.83)$ \\
%             & $224^{2}$ & $70.24$ & $72.02$ & $18.80$ & $37.78$ & $19.08$ & $64.31$ & $61.11$  & $47.75$ & $79.04$ & $49.99 (\pm21.62)$ \\
%      %\hline %%%%%%%%%%%%%%%%%%%%%%%
%      VGGm-11 & $32^{2}$ & $63.74$ & $62.59$ & $18.62$ & $26.27$ & $14.49$ & $56.47$ & $49.88$  & $47.67$ & $76.86$ & $44.11 (\pm20.79)$ \\
%             & $224^{2}$ & $83.02$ & $70.49$ & $24.17$ & $33.09$ & $28.62$ & $70.59$ & $68.03$  & $50.92$ & $85.43$ & $53.92 (\pm21.54)$ \\
%      VGGm-17 & $32^{2}$ & $65.78$ & $53.06$ & $12.13$ & $16.34$ & $7.98$ & $40.88$ & $46.55$ & $37.01$  & $74.39$ & $36.04 (\pm21.34)$ \\
%             & $224^{2}$ & $86.28$ & $71.68$ & $22.62$ & $28.65$ & $22.59$ & $64.12$ & $69.80$ & $50.45$  & $85.39$ & $51.91 (\pm23.03)$ \\
%      ResNet-18 & $32^{2}$ & $49.70$ & $51.19$ & $13.17$ & $19.61$ & $11.49$ & $39.22$ & $36.47$ & $41.75$  & $65.91$ & $34.85 (\pm17.85)$ \\
%                & $224^{2}$ & $81.74$ & $70.32$ & $27.68$ & $34.47$ & $21.33$ & $62.55$ & $68.63$ & $57.27$  & $84.68$ & $53.37 (\pm21.34)$ \\
%      %%%%%%
%      ResNet-34 & $32^{2}$ & $50.80$ & $49.57$ & $12.10$ & $18.28$ & $10.44$ & $37.84$  & $35.05$& $39.39$  & $66.08$ & $33.59 (\pm18.02)
% $ \\
%                & $224^{2}$ & $83.12$ & $70.83$ & $23.27$ & $30.79$ & $22.62$ & $58.24$ & $66.99$ & $52.61$  & $83.79$ & $51.14 (\pm21.68)$ \\

ViT-T & $32^{2}$ & $-3.29\%$ & $3.74\%$ & $2.32\%$ & $3.08\%$ & $-4.97\%$ & $5.23\%$ & $-8.04\%$ & $1.46\%$ & $-0.74\%$& $0.26(\pm4.30)$ \\
ViT-T & $224^{2}$ & $-2.85\%$ & $22.66\%$ & $55.11\%$ & $118.64\%$ & $86.23\%$ & $130.00\%$ & $28.36\%$ & $31.05\%$ & $13.75\%$& $60.72(\pm42.45)$ \\
ViT-T+ & $32^{2}$ & $15.43\%$ & $15.85\%$ & $24.06\%$ & $27.11\%$ & $4.64\%$ & $19.56\%$ & $21.18\%$ & $17.49\%$ & $7.91\%$& $17.23(\pm7.18)$ \\
ViT-T+ & $224^{2}$ & $18.29\%$ & $42.36\%$ & $116.59\%$ & $216.42\%$ & $170.64\%$ & $195.54\%$ & $80.69\%$ & $58.16\%$ & $32.15\%$& $114.07(\pm67.46)$ \\
VGGm-11 & $32^{2}$ & $22.06\%$ & $21.46\%$ & $22.34\%$ & $49.09\%$ & $-11.21\%$ & $38.47\%$ & $25.71\%$ & $9.81\%$ & $11.62\%$& $20.91(\pm17.21)$ \\
VGGm-11 & $224^{2}$ & $5.44\%$ & $17.92\%$ & $27.08\%$ & $86.11\%$ & $62.24\%$ & $68.23\%$ & $6.53\%$ & $32.09\%$ & $10.09\%$& $38.79(\pm27.70)$ \\
VGGm-17 & $32^{2}$ & $26.45\%$ & $66.86\%$ & $43.89\%$ & $135.45\%$ & $100.00\%$ & $172.53\%$ & $65.84\%$ & $52.87\%$ & $23.12\%$& $82.57(\pm46.95)$ \\
VGGm-17 & $224^{2}$ & $7.47\%$ & $41.91\%$ & $29.11\%$ & $135.80\%$ & $137.54\%$ & $146.81\%$ & $31.33\%$ & $56.19\%$ & $9.56\%$& $73.53(\pm53.02)$ \\
ResNet-18 & $32^{2}$ & $44.56\%$ & $107.58\%$ & $131.87\%$ & $338.70\%$ & $136.42\%$ & $303.91\%$ & $116.18\%$ & $108.23\%$ & $35.37\%$& $159.78(\pm98.03)$ \\
ResNet-18 & $224^{2}$ & $18.81\%$ & $28.20\%$ & $47.23\%$ & $63.68\%$ & $23.44\%$ & $43.04\%$ & $28.81\%$ & $48.52\%$ & $13.73\%$& $37.08(\pm15.23)$ \\
ResNet-34 & $32^{2}$ & $58.26\%$ & $103.16\%$ & $191.57\%$ & $286.47\%$ & $112.20\%$ & $297.90\%$ & $157.15\%$ & $112.92\%$ & $44.88\%$& $163.28(\pm84.35)$ \\
ResNet-34 & $224^{2}$ & $20.71\%$ & $33.69\%$ & $54.93\%$ & $80.90\%$ & $50.50\%$ & $81.66\%$ & $34.60\%$ & $57.14\%$ & $16.54\%$& $51.24(\pm21.34)$ \\
     \hline
    \end{tabular}}
  \label{tab:acc_ood_transfer}
\end{table}

==> tables/aug_table.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Augmentation reduces the tunnel effect.} We report average results with 95\% confidence intervals (CI). %for various resolutions and metrics. 
Mean effect (ME) shows the average difference in performance between no augmentation and augmentation, demonstrating how performance changes as augmentation is used. There are no ME values for augmentation as it is used as the reference point for comparison.}

\label{tab:aug_no_aug_comp}
\resizebox{\textwidth}{!}{\begin{tabular}{c|cccc|cccc|cccc}
\hline
 & \multicolumn{4}{c|}{\textbf{\% OOD Performance Retained $\uparrow$}} & \multicolumn{4}{c|}{\textbf{Pearson Correlation $\uparrow$}} & \multicolumn{4}{c}{\textbf{ID/OOD Alignment $\uparrow$}} \\
& Avg. & CI & ME & ME CI & Avg. & CI & ME & ME CI & Avg. & CI & ME & ME CI \\

\hline   
No Aug. & $64.26$ & $61.20$--$67.31$ & $14.15$ & $12.28$--$16.02$ & $0.77$ & $0.74$--$0.80$ & $0.09$ & $0.08$--$0.11$ & $0.15$ & $0.14$--$0.17$ & $0.09$ & $0.08$--$0.10$ \\
\textbf{Aug.} & $\mathbf{78.41}$ & $\mathbf{75.65}$--$\mathbf{81.16}$ & \textit{N/A} & \textit{N/A} & $\mathbf{0.86}$ & $\mathbf{0.84}$--$\mathbf{0.89}$ & \textit{N/A} & \textit{N/A} & $\mathbf{0.25}$ & $\mathbf{0.23}$--$\mathbf{0.27}$ & \textit{N/A} & \textit{N/A} \\
\hline
\end{tabular}}
\end{table}

==> tables/cl_exp.tex <==
\begin{table}[t]
\centering
  \caption{\textbf{Continual Learning Results}. %The tunnel part is task-specific and impacts forgetting.
  The ResNet-18 is subsequently trained on two tasks. Each task consists of 50 ImageNet classes. $E_{t}$ and $T_{t}$ denote extractor and tunnel respectively for tasks $t \in \{1, 2\}$. Reported is top-1 accuracy (\%) on the test set of the corresponding task. Here \textcolor{red}{red} and \textcolor{blue}{blue} indicate degraded and maximally enhanced accuracy respectively. Bold indicates original task accuracy. Finetuning (abbreviated as FT) has been performed to recover 1st task performance, therefore 2nd task columns are empty. %\yh{we may wrap the table around text to gain space.}
  %\ck{You have to explain why there are dashes} \yh{done}
  } 
  \label{tab:cl_exp}
  \centering
     \begin{tabular}{c|ccc}
     \hline \hline
      Resolution & Combination & 1st Task $\uparrow$ & 2nd Task $\uparrow$ \\
     \hline \hline    
     & $E_{1} + T_{1}$ & $\mathbf{64.04}$ & $21.20$ \\
     & $E_{1} + T_{2}$ & \color{red}{$37.64$} & $35.64$ \\
     $32\times32$ & $E_{2} + T_{2}$ & $20.44$ & $\mathbf{68.16}$ \\
     & $E_{2} + T_{1}$ & $29.84$ & \color{red}{$23.84$} \\
     \cline{2-4}
     & $E_{2} + T_{1} (FT)$ & \color{blue}{$51.40$} & -- \\
     & $E_{2} (FT)$ & $45.60$ & -- \\
    \hline
     & $E_{1} + T_{1}$ & $\mathbf{74.36}$ & $23.24$ \\
     & $E_{1} + T_{2}$ & \color{red}{$54.32$} & $35.68$ \\
     $224\times224$ & $E_{2} + T_{2}$ & $20.44$ & $\mathbf{78.00}$ \\
     & $E_{2} + T_{1}$ & $21.56$ & \color{red}{$46.08$} \\
     \cline{2-4}
     & $E_{2} + T_{1} (FT)$ & \color{blue}{$57.24$} & -- \\
     & $E_{2} (FT)$ & $52.48$ & -- \\
    \hline \hline
    %\vspace{-2em}
    \end{tabular}
\end{table}


==> tables/correlations_cifar10.tex <==


\begin{table}[t!]
  \caption{\textbf{Pearson correlation.} Correlation between OOD and ID linear probes based on top-1 accuracy on the corresponding test dataset. CIFAR-10 is ID dataset}
  \centering
  \resizebox{\linewidth}{!}{
  \begin{tabular}{l|cccccccc|c}
     \hline
     \multicolumn{1}{c}{\textbf{Model}} &

     \multicolumn{9}{c}{\textbf{Correlation}} \\
   &\textbf{NINCO} & \textbf{ImageNet-R} & \textbf{CUB} & \textbf{Aircrafts} & \textbf{Flowers} & \textbf{Pets} & \textbf{CIFAR}  & \textbf{STL} & \textbf{Avg. ($\pm$ Std.)} \\ 
     \hline
     \textcolor{orange}{\emph{\textbf{No Aug}}}  & & & & & & & & & \\
    VGGm-11 & 0.38 & 0.53 & 0.33 & 0.47 & 0.36 & 0.58 & 0.59 & 0.99 & 0.53 (\pm 0.20) \\
VGGm-17 & -0.03 & 0.19 & -0.05 & 0.15 & -0.04 & 0.18 & 0.11 & 0.97 & 0.18 (\pm 0.31) \\



     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
     \hline
     \textcolor{orange}{\emph{\textbf{Aug}}}  & & & & & & & & & \\

     \hline
    \end{tabular}}
  \label{tab:acc_ood_transfer}
\end{table}

==> tables/correlations_cifar100.tex <==


\begin{table}[t!]
  \caption{\textbf{Pearson correlation.} Correlation between OOD and ID linear probes based on top-1 accuracy on the corresponding test dataset. CIFAR-100 is ID dataset}
  \centering
  \resizebox{\linewidth}{!}{
  \begin{tabular}{l|cccccccc|c}
     \hline
     \multicolumn{1}{c}{\textbf{Model}} &

     \multicolumn{9}{c}{\textbf{Correlation}} \\
   &\textbf{NINCO} & \textbf{ImageNet-R} & \textbf{CUB} & \textbf{Aircrafts} & \textbf{Flowers} & \textbf{Pets} & \textbf{CIFAR}  & \textbf{STL} & \textbf{Avg. ($\pm$ Std.)} \\ 
     \hline
     \textcolor{orange}{\emph{\textbf{No Aug}}}  & & & & & & & & & \\
VGGm-11 & 0.91 & 0.91 & 0.72 & 0.84 & 0.81 & 0.88 & 0.94 & 0.93 & 0.87 (\pm 0.07)\\
VGGm-17 & 0.56 & 0.49 & 0.23 & 0.34 & 0.26 & 0.53 & 0.65 & 0.66 & 0.46 (\pm 0.16)\\



     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
     \hline
     \textcolor{orange}{\emph{\textbf{Aug}}}  & & & & & & & & & \\
VGGm$\dag$-11 & 0.96 & 0.99 & 0.95 & 0.94 & 0.97 & 0.97 & 0.96 & 0.97 & 0.96 (\pm 0.01)\\
VGGm$\dag$-17 & 0.89 & 0.95 & 0.84 & 0.75 & 0.80 & 0.91 & 0.93 & 0.91 & 0.87 (\pm 0.06)\\
     \hline
    \end{tabular}}
  \label{tab:acc_ood_transfer}
\end{table}

==> tables/pearson_corr.tex <==


\begin{table}[t!]
  \caption{\textbf{Pearson correlation.} Correlation between OOD and ID linear probes based on top-1 accuracy on the corresponding test dataset. VGGm$\dag$ denotes VGGm without max-pool in the first two stages for $32\times 32$ input resolution only.}
  \centering
  \resizebox{\linewidth}{!}{
  \begin{tabular}{lcc|cccccccc|c}
     \hline
     \multicolumn{1}{c}{\textbf{Model}} &
     \multicolumn{1}{c}{\textbf{\gamma}} &
     \multicolumn{1}{c|}{\textbf{Image}} &
     \multicolumn{9}{c}{\textbf{Correlation}} \\
      & & \textbf{Size} &\textbf{NINCO} & \textbf{ImageNet-R} & \textbf{CUB} & \textbf{Aircrafts} & \textbf{Flowers} & \textbf{Pets} & \textbf{CIFAR}  & \textbf{STL} & \textbf{Avg. ($\pm$ Std.)} \\
     \hline
     \textcolor{orange}{\emph{\textbf{No Aug}}} & & & & & & & & & & & \\
VGGm$\dag$-11 & 74.67 & $32^2$ & $0.93$  & $0.98$  & $0.88$  & $0.91$  & $0.87$  & $0.98$  & $0.93$  & $0.97$  & $0.93(\pm0.04)$ \\
VGGm-11 & 74.67 & $32^2$ & $0.96$  & $0.93$  & $0.85$  & $0.85$  & $0.87$  & $0.98$  & $0.92$  & $0.95$  & $0.91(\pm0.05)$ \\
VGGm-11 & 74.67 & $224^2$ & $0.92$  & $0.97$  & $0.86$  & $0.88$  & $0.81$  & $0.99$  & $0.92$  & $0.96$  & $0.91(\pm0.06)$ \\
VGGm$\dag$-17 & 158.5 & $32^2$ & $0.84$  & $0.94$  & $0.76$  & $0.71$  & $0.70$  & $0.96$  & $0.87$  & $0.95$  & $0.84(\pm0.1)$ \\
VGGm-17 & 158.5 & $32^2$ & $0.62$  & $0.61$  & $0.38$  & $0.38$  & $0.35$  & $0.88$  & $0.55$  & $0.86$  & $0.58(\pm0.19)$ \\
VGGm-17 & 158.5 & $224^2$ & $0.84$  & $0.92$  & $0.69$  & $0.66$  & $0.62$  & $0.97$  & $0.84$  & $0.95$  & $0.81(\pm0.13)$ \\
ViT-T & 44.28 & $32^2$ & $0.94$  & $0.97$  & $0.97$  & $0.96$  & $0.94$  & $0.99$  & $0.97$  & $0.96$  & $0.96(\pm0.02)$ \\
ViT-T & 44.28 & $224^2$ & $0.75$  & $0.70$  & $0.53$  & $0.55$  & $0.40$  & $0.90$  & $0.61$  & $0.83$  & $0.66(\pm0.16)$ \\
ViT-T+ & 66.23 & $32^2$ & $0.95$  & $0.95$  & $0.93$  & $0.87$  & $0.88$  & $0.97$  & $0.97$  & $0.95$  & $0.94(\pm0.04)$ \\
ViT-T+ & 66.23 & $224^2$ & $0.68$  & $0.59$  & $0.46$  & $0.47$  & $0.42$  & $0.83$  & $0.62$  & $0.74$  & $0.60(\pm0.14)$ \\
ResNet-18 & 88.56 & $32^2$ & $0.83$  & $0.76$  & $0.69$  & $0.71$  & $0.68$  & $0.90$  & $0.77$  & $0.92$  & $0.78(\pm0.09)$ \\
ResNet-18 & 88.56 & $224^2$ & $0.97$  & $0.97$  & $0.96$  & $0.93$  & $0.97$  & $0.98$  & $0.96$  & $0.99$  & $0.96(\pm0.02)$ \\
ResNet-34 & 168.37 & $32^2$ & $0.78$  & $0.68$  & $0.58$  & $0.62$  & $0.48$  & $0.83$  & $0.72$  & $0.87$  & $0.69(\pm0.12)$ \\
ResNet-34 & 168.37 & $224^2$ & $0.87$  & $0.90$  & $0.84$  & $0.81$  & $0.74$  & $0.98$  & $0.79$  & $0.91$  & $0.86(\pm0.07)$ \\
     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
     \hline
     \textcolor{orange}{\emph{\textbf{Aug}}} & & & & & & & & & & & \\
VGGm$\dag$-11 & 74.67 & $32^2$ & $0.95$  & $0.99$  & $0.98$  & $0.95$  & $0.94$  & $0.99$  & $0.95$  & $0.95$  & $0.96(\pm0.02)$ \\
VGGm-11 & 74.67 & $32^2$ & $0.97$  & $0.95$  & $0.94$  & $0.78$  & $0.93$  & $0.99$  & $0.92$  & $0.97$  & $0.93(\pm0.06)$ \\
VGGm-11 & 74.67 & $224^2$ & $0.96$  & $0.99$  & $0.98$  & $0.95$  & $0.95$  & $0.99$  & $0.97$  & $0.97$  & $0.97(\pm0.01)$ \\
VGGm$\dag$-17 & 158.5 & $32^2$ & $0.94$  & $0.96$  & $0.94$  & $0.78$  & $0.90$  & $0.99$  & $0.94$  & $0.97$  & $0.93(\pm0.06)$ \\
VGGm-17 & 158.5 & $32^2$ & $0.85$  & $0.62$  & $0.60$  & $0.30$  & $0.64$  & $0.97$  & $0.62$  & $0.93$  & $0.69(\pm0.2)$ \\
VGGm-17 & 158.5 & $224^2$ & $0.95$  & $0.97$  & $0.94$  & $0.86$  & $0.91$  & $0.99$  & $0.95$  & $0.96$  & $0.94(\pm0.04)$ \\
ViT-T & 44.28 & $32^2$ & $0.96$  & $0.99$  & $0.99$  & $0.95$  & $0.97$  & $0.99$  & $0.99$  & $0.99$  & $0.98(\pm0.02)$ \\
ViT-T & 44.28 & $224^2$ & $0.95$  & $0.99$  & $0.98$  & $0.98$  & $0.98$  & $0.99$  & $0.95$  & $0.98$  & $0.97(\pm0.02)$ \\
ViT-T+ & 66.23 & $32^2$ & $0.96$  & $0.99$  & $0.98$  & $0.96$  & $0.97$  & $1.00$  & $0.99$  & $0.99$  & $0.98(\pm0.01)$ \\
ViT-T+ & 66.23 & $224^2$ & $0.97$  & $0.98$  & $0.98$  & $0.98$  & $0.96$  & $0.99$  & $0.94$  & $0.98$  & $0.97(\pm0.01)$ \\
ResNet-18 & 88.56 & $32^2$ & $0.96$  & $0.90$  & $0.91$  & $0.83$  & $0.92$  & $0.98$  & $0.91$  & $0.96$  & $0.92(\pm0.04)$ \\
ResNet-18 & 88.56 & $224^2$ & $0.98$  & $0.98$  & $0.97$  & $0.95$  & $0.99$  & $0.97$  & $0.99$  & $0.99$  & $0.98(\pm0.01)$ \\
ResNet-34 & 168.37 & $32^2$ & $0.90$  & $0.81$  & $0.79$  & $0.41$  & $0.77$  & $0.98$  & $0.82$  & $0.92$  & $0.80(\pm0.16)$ \\
ResNet-34 & 168.37 & $224^2$ & $0.93$  & $0.96$  & $0.95$  & $0.84$  & $0.87$  & $0.99$  & $0.94$  & $0.94$  & $0.93(\pm0.05)$ \\

     \hline
    \end{tabular}}
  \label{tab:pearson_corr}
\end{table}

==> tables/resolution_ood_result.tex <==
\begin{table}[t]
\centering
  \caption{\textbf{Spearman Correlation and NC1.} Spearman correlation ($\rho$) between OOD and ID test accuracy across layers of VGG-11 with different image resolutions. The VGG-11 is trained on ImageNet-100 (ID dataset) and evaluated on Places and NINCO (OOD datasets). NC1 is evaluated using ID dataset. \ck{Table 1 and Table 2 should be combined -- all of the models we trained in a controlled manner where we controlled the resolution should be in a single table, where we use rho, NC1, and NC4}
  } 
  \label{tab:resolution_ood_result}
  \centering
     \begin{tabular}{cccc}
     \hline
   Resolution & $\rho$ (Places) $\uparrow$ & $\rho$ (NINCO) $\uparrow$ & NC1 $\uparrow$ \\
     \hline   
    $32\times32$   & $0.600$ & $0.503$ & $0.105$ \\
    $64\times64$   & $0.988$ & $0.976$ &  $0.261$ \\
    $128\times128$ & $\mathbf{0.999}$ & $\mathbf{0.999}$ &  $0.469$ \\
    $224\times224$ & $\mathbf{0.999}$ & $\mathbf{0.999}$ &  $\mathbf{0.568}$\\
    \hline
    %\vspace{-2em}
    \end{tabular}
\end{table}



==> tables/summary_table.tex <==
\begin{table}[t!]
  \caption{\textbf{Summary of the tunnel effect findings.} We report the magnitude of the tunnel effect in terms of average $\%$ drop in OOD linear probe accuracy across OOD datasets from the layer with the highest accuracy to the final layer. For each OOD dataset, we measure the $\%$ OOD degradation and finally report the average $\%$ OOD degradation over all OOD datasets. A lower value (bold) indicates a weaker tunnel effect (i.e., better transfer to OOD datasets) and vice-versa. 
  %VGGm denotes modified VGG without two FC layers before the final layer. VGGm$\dag$ denotes VGGm without max-pool in the first two stages for $32\times 32$ input resolution only.
  NA means not applicable.
   }
  \centering
  \resizebox{\linewidth}{!}{
  \begin{tabular}{cccccccccc}
     \hline
     \multicolumn{1}{c}{\textbf{Resolution}} &
     \multicolumn{8}{c}{\textbf{Model}} &
     \multicolumn{1}{c}{\textbf{Avg. ($\pm$ Std.)}} \\
     %\cline{2-7}
      & \textbf{ViT-T} & \textbf{ViT-T+} & \textbf{VGGm-11} & \textbf{VGGm-17} & \textbf{VGGm$\dag$-11} & \textbf{VGGm$\dag$-17} & \textbf{ResNet-18} & \textbf{ResNet-34} & \\
     %& \textbf{\rotatebox[origin=c]{45}{ViT-T}} & \textbf{\rotatebox[origin=c]{45}{ViT-T+}} & \textbf{\rotatebox[origin=c]{45}{VGGm-11}} & \textbf{\rotatebox[origin=c]{45}{VGGm-17}} & \textbf{\rotatebox[origin=c]{45}{VGGm$\dag$-11}} & \textbf{\rotatebox[origin=c]{45}{VGGm$\dag$-17}} & \textbf{\rotatebox[origin=c]{45}{ResNet-18}} & \textbf{\rotatebox[origin=c]{45}{ResNet-34}} & \\
     \hline
     \textcolor{orange}{\emph{\textbf{No Aug}}} & & & & & & & & & \\
     $32^{2}$ & $\mathbf{5.02}$ & $\mathbf{7.70}$ & $21.37$ & $53.85$ & $\mathbf{12.74}$ & $\mathbf{35.03}$ & $58.71$ & $61.48$ & $34.69 (\pm23.97)$ \\
     $224^{2}$ & $37.32$ & $45.35$ & $\mathbf{14.30}$ & $\mathbf{36.17}$ & NA & NA & $\mathbf{19.21}$ & $\mathbf{35.14}$ & $\mathbf{31.25} (\pm10.86)$ \\
     \hline
     \textcolor{orange}{\emph{\textbf{Aug}}} & & & & & & & & & \\
     $32^{2}$ & $\mathbf{4.61}$ & $\mathbf{5.76}$ & $13.06$ & $34.00$ & $\mathbf{1.02}$ & $\mathbf{13.56}$ & $28.17$ & $31.45$ & $19.51 (\pm12.11)$ \\
     $224^{2}$ & $6.95$ & $7.33$ & $\mathbf{2.39}$ & $\mathbf{10.94}$ & NA & NA & $\mathbf{11.80}$ & $\mathbf{20.79}$ & $\mathbf{10.03} (\pm5.70)$ \\
     \hline
    \end{tabular}}
  \label{tab:summary_table}
\end{table}

==> tables/variables_comparison_summary.tex <==
\begin{table}[t]
\centering
\caption{
}

\label{tab:variable_comparison}
\resizebox{\textwidth}{!}{\begin{tabular}{c|cc|cc|cc|c}
\textbf{Comparisons} & \multicolumn{2}{c|}{\textbf{\% OOD Performance Retained}} & \multicolumn{2}{c|}{\textbf{Pearson Correlation}} & \multicolumn{2}{c}{\textbf{ID/OOD Alignment}} \\
 & Mean Effect $\uparrow$ & $p-$value $\downarrow$ & Mean Effect $\uparrow$ & $p-$value $\downarrow$ & Mean Effect $\uparrow$ & $p-$value $\downarrow$ &\textbf{\#}\\
 \hline
 \textcolor{orange}{\emph{\textbf{Resolution}}} & & & & & & \\
$32^2$ vs $64^2$ & $1.15$ & $0.742$ & $0.02$ & $0.490$ & $0.08$ & $p<0.001$ & 48 \\
$32^2$ vs $128^2$ & $8.61$ & $p<0.001$ & $0.06$ & $0.014$ & $0.15$ & $p<0.001$ & 48 \\
$32^2$ vs $224^2$ & $9.74$ & $0.013$ & $0.06$ & $0.056$ & $0.18$ & $p<0.001$ & 48 \\
$64^2$ vs $128^2$ & $7.46$ & $p<0.001$ & $0.05$ & $p<0.001$ & $0.07$ & $p<0.001$ & 48 \\
$64^2$ vs $224^2$ & $8.59$ & $p<0.001$ & $0.05$ & $0.163$ & $0.10$ & $p<0.001$ & 48 \\
$128^2$ vs $224^2$ & $1.13$ & $0.624$ & $0.00$ & $0.989$ & $0.03$ & $0.016$ & 48 \\
\hline
\textcolor{orange}{\emph{\textbf{Augmentation}}} & & & & & & \\
Off vs On & $14.15$ & $p<0.001$ & $0.09$ & $p<0.001$ & $0.09$ & $p<0.001$ & 256 \\
\hline
\textcolor{orange}{\emph{\textbf{Stem}}} & & & & & & \\
$3$ vs $7$ & $10.08$ & $p<0.001$ & $0.02$ & $0.069$ & $0.06$ & $p<0.001$ & 64 \\
$3$ vs $8$ & $8.62$ & $0.005$ & $0.04$ & $0.171$ & $0.10$ & $p<0.001$ & 64 \\
$7$ vs $8$ & $18.70$ & $p<0.001$ & $0.02$ & $0.520$ & $0.04$ & $p<0.001$ & 64 \\
\hline
\textcolor{orange}{\emph{\textbf{Spatial Reduction}}} & & & & & & \\
$1$ vs $0.5$ & $14.99$ & $p<0.001$ & $0.14$ & $p<0.001$ & $0.08$ & $p<0.001$ & 32 \\
\hline
\textcolor{orange}{\emph{\textbf{Depth}}} & & & & & & \\
$11$ vs $12$ & $0.23$ & $0.942$ & $0.04$ & $0.141$ & $0.12$ & $p<0.001$ & 32 \\
$11$ vs $17$ & $20.96$ & $p<0.001$ & $0.18$ & $p<0.001$ & $0.04$ & $p<0.001$ & 32 \\
$11$ vs $18(ResNet-18)$ & $16.69$ & $p<0.001$ & $0.02$ & $0.147$ & $0.07$ & $p<0.001$ & 32 \\
$11$ vs $18(ViT-T+)$ & $3.50$ & $0.323$ & $0.06$ & $0.041$ & $0.11$ & $p<0.001$ & 32 \\
$11$ vs $34$ & $24.43$ & $p<0.001$ & $0.11$ & $p<0.001$ & $0.09$ & $p<0.001$ & 32 \\
$12$ vs $17$ & $20.73$ & $p<0.001$ & $0.14$ & $0.005$ & $0.09$ & $p<0.001$ & 32 \\
$12$ vs $18(ResNet-18)$ & $16.46$ & $0.003$ & $0.02$ & $0.624$ & $0.05$ & $0.001$ & 32 \\
$12$ vs $18(ViT-T+)$ & $3.27$ & $p<0.001$ & $0.02$ & $0.002$ & $0.01$ & $0.076$ & 32 \\
$12$ vs $34$ & $24.20$ & $p<0.001$ & $0.07$ & $0.057$ & $0.04$ & $0.015$ & 32 \\
$17$ vs $18(ResNet-18)$ & $4.27$ & $0.058$ & $0.16$ & $p<0.001$ & $0.03$ & $0.003$ & 32 \\
$17$ vs $18(ViT-T+)$ & $17.46$ & $p<0.001$ & $0.12$ & $0.018$ & $0.07$ & $p<0.001$ & 32 \\
$17$ vs $34$ & $3.47$ & $0.028$ & $0.06$ & $p<0.001$ & $0.05$ & $p<0.001$ & 32 \\
$18(ResNet-18)$ vs $18(ViT-T+)$ & $13.19$ & $0.020$ & $0.04$ & $0.307$ & $0.04$ & $0.002$ & 32 \\
$18(ResNet-18)$ vs $34$ & $7.74$ & $p<0.001$ & $0.09$ & $p<0.001$ & $0.02$ & $p<0.001$ & 32 \\
$18(ViT-T+)$ vs $34$ & $20.94$ & $p<0.001$ & $0.05$ & $0.190$ & $0.02$ & $0.038$ & 32 \\
\hline
\textcolor{orange}{\emph{\textbf{Overparam Level}}} & & & & & & \\
$44.28$ vs $66.23$ & $3.27$ & $p<0.001$ & $0.02$ & $0.002$ & $0.01$ & $0.076$ & 32 \\
$44.28$ vs $74.67$ & $0.23$ & $0.942$ & $0.04$ & $0.141$ & $0.12$ & $p<0.001$ & 32 \\
$44.28$ vs $88.56$ & $16.46$ & $0.003$ & $0.02$ & $0.624$ & $0.05$ & $0.001$ & 32 \\
$44.28$ vs $158.5$ & $20.73$ & $p<0.001$ & $0.14$ & $0.005$ & $0.09$ & $p<0.001$ & 32 \\
$44.28$ vs $168.37$ & $24.20$ & $p<0.001$ & $0.07$ & $0.057$ & $0.04$ & $0.015$ & 32 \\
$66.23$ vs $74.67$ & $3.50$ & $0.323$ & $0.06$ & $0.041$ & $0.11$ & $p<0.001$ & 32 \\
$66.23$ vs $88.56$ & $13.19$ & $0.020$ & $0.04$ & $0.307$ & $0.04$ & $0.002$ & 32 \\
$66.23$ vs $158.5$ & $17.46$ & $p<0.001$ & $0.12$ & $0.018$ & $0.07$ & $p<0.001$ & 32 \\
$66.23$ vs $168.37$ & $20.94$ & $p<0.001$ & $0.05$ & $0.190$ & $0.02$ & $0.038$ & 32 \\
$74.67$ vs $88.56$ & $16.69$ & $p<0.001$ & $0.02$ & $0.147$ & $0.07$ & $p<0.001$ & 32 \\
$74.67$ vs $158.5$ & $20.96$ & $p<0.001$ & $0.18$ & $p<0.001$ & $0.04$ & $p<0.001$ & 32 \\
$74.67$ vs $168.37$ & $24.43$ & $p<0.001$ & $0.11$ & $p<0.001$ & $0.09$ & $p<0.001$ & 32 \\
$88.56$ vs $158.5$ & $4.27$ & $0.058$ & $0.16$ & $p<0.001$ & $0.03$ & $0.003$ & 32 \\
$88.56$ vs $168.37$ & $7.74$ & $p<0.001$ & $0.09$ & $p<0.001$ & $0.02$ & $p<0.001$ & 32 \\
$158.5$ vs $168.37$ & $3.47$ & $0.028$ & $0.06$ & $p<0.001$ & $0.05$ & $p<0.001$ & 32 \\
\hline
\textcolor{orange}{\emph{\textbf{ID Dataset}}} & & & & & & \\
Imagenet-100 vs Cifar-10 & $46.97$ & $p<0.001$ & $0.38$ & $p<0.001$ & $0.09$ & $0.004$ & 16 \\
Imagenet-100 vs Cifar-100 & $9.36$ & $0.001$ & $0.04$ & $0.008$ & $0.00$ & $0.908$ & 16 \\
Cifar-10 vs Cifar-100 & $37.61$ & $p<0.001$ & $0.35$ & $p<0.001$ & $0.10$ & $0.005$ & 16 \\
\hline
\textcolor{orange}{\emph{\textbf{Sample Class}}} & & & & & & \\
C10\_S1000 vs C50\_S200 & $39.11$ & $p<0.001$ & $0.41$ & $p<0.001$ & $0.05$ & $p<0.001$ & 16 \\
C10\_S1000 vs C100\_S100 & $49.96$ & $p<0.001$ & $0.48$ & $p<0.001$ & $0.02$ & $p<0.001$ & 16 \\
C10\_S1000 vs C100\_S200 & $44.67$ & $p<0.001$ & $0.46$ & $p<0.001$ & $0.05$ & $p<0.001$ & 16 \\
C10\_S1000 vs C100\_S500 & $48.43$ & $p<0.001$ & $0.48$ & $p<0.001$ & $0.12$ & $p<0.001$ & 16 \\
C10\_S1000 vs C100\_S700 & $47.58$ & $p<0.001$ & $0.48$ & $p<0.001$ & $0.13$ & $p<0.001$ & 16 \\
C50\_S200 vs C100\_S100 & $10.85$ & $p<0.001$ & $0.07$ & $p<0.001$ & $0.03$ & $p<0.001$ & 16 \\
C50\_S200 vs C100\_S200 & $5.55$ & $p<0.001$ & $0.05$ & $p<0.001$ & $0.00$ & $0.383$ & 16 \\
C50\_S200 vs C100\_S500 & $9.31$ & $p<0.001$ & $0.06$ & $p<0.001$ & $0.07$ & $p<0.001$ & 16 \\
C50\_S200 vs C100\_S700 & $8.47$ & $p<0.001$ & $0.07$ & $p<0.001$ & $0.08$ & $p<0.001$ & 16 \\
C100\_S100 vs C100\_S200 & $5.29$ & $0.001$ & $0.02$ & $0.097$ & $0.03$ & $p<0.001$ & 16 \\
C100\_S100 vs C100\_S500 & $1.54$ & $0.323$ & $0.00$ & $0.839$ & $0.09$ & $p<0.001$ & 16 \\
C100\_S100 vs C100\_S700 & $2.38$ & $0.212$ & $0.00$ & $0.894$ & $0.11$ & $p<0.001$ & 16 \\
C100\_S200 vs C100\_S500 & $3.76$ & $0.003$ & $0.02$ & $0.046$ & $0.07$ & $p<0.001$ & 16 \\
C100\_S200 vs C100\_S700 & $2.91$ & $0.049$ & $0.02$ & $0.028$ & $0.08$ & $p<0.001$ & 16 \\
C100\_S500 vs C100\_S700 & $0.84$ & $0.167$ & $0.01$ & $0.152$ & $0.02$ & $p<0.001$ & 16 \\
\hline
\hline
\end{tabular}}
\end{table}

==> tables/vgg_classes_samples_id.tex <==
\begin{table}[h]
\centering
\caption{ID performance of VGGm-11 trained on ImageNet-100 ($32\times 32$) using specified classes and samples per class, with and without augmentation. Reported is the best top-1 accuracy (\%).}
\label{tab:vgg_samples_classes_id_acc}

\begin{tabular}{c | c c c | c c c}
\hline
\multicolumn{1}{c|}{\textbf{Model}} & \multicolumn{3}{c|}{\textbf{Aug}} & \multicolumn{3}{c}{\textbf{No Aug}} \\
 & \# Class & \# Sample & Accuracy & \# Class & \# Sample & Accuracy \\
\hline
 & 10 & 1000 & 77.0 & 10 & 1000 & 70.2 \\
%VGGm-17 & 10 & 1000 & 78.0 & 10 & 1000 & 65.6 \\
%\hline
 & 50 & 200 & 50.7 & 50 & 200 & 37.2 \\
%VGGm-17 & 50 & 200 & 52.2 & 50 & 200 & 29.8 \\
%\hline
VGGm-11 & 100 & 100 & 33.2 & 100 & 100 & 26.1 \\
%VGGm-17 & 100 & 100 & 32.5 & 100 & 100 & 18 \\
%\hline
 & 100 & 200 & 45.0 & 100 & 200 & 32.8 \\
%VGGm-17 & 100 & 200 & 41.3 & 100 & 200 & 27.6 \\
%\hline
 & 100 & 500 & 57.1 & 100 & 500 & 44.7 \\
%VGGm-17 & 100 & 500 & 60.2 & 100 & 500 & 41.1 \\
%\hline
 & 100 & 700 & 61.6 & 100 & 700 & 47.5 \\
%VGGm-17 & 100 & 700 & 63.6 & 100 & 700 & 45.2 \\
\hline
\end{tabular}
\end{table}
